Characterization of Maximizers in A Non-Convex Geometric Optimization Problem With Application to Optical Wireless Power Transfer Systems

This research studies a non-convex geometric optimization problem arising from the field of optical wireless power transfer. In the considered optimization problem, the cost function is a sum of negatively and fractionally powered distances from given points arbitrarily located in a plane to another point belonging to a different plane. Therefore, it is a strongly nonlinear and non-convex programming, hence posing a challenge on the characterization of its optimizer set, especially its set of global optimizers. To tackle this challenge, the bifurcation theory is employed to investigate the continuation and bifurcation structures of the Hessian matrix of the cost function. As such, two main results are derived. First, there is a critical distance between the two considered planes such that beyond which a unique global optimizer exists. Second, the exact number of maximizers is locally derived by the number of bifurcation branches determined via one-dimensional isotropic subgroups of a Lie group acting on $\mathbb{R}^2$, when the inter-plane distance is smaller than the above-mentioned critical distance. Consequently, numerical simulations and computations of bifurcation points are carried out for various configurations of the given points, whose results confirm the derived theoretical outcomes.

==> Hoa_maximizer.tex <==
 %% !TEX encoding = UTF-8 Unicode
%\documentclass{article}
%%\documentclass[draft]{article}
%\usepackage{authblk}
%\usepackage{fancyhdr}
%\usepackage{amscd}
%%\usepackage{graphicx}
%%\usepackage[dvipdfm]{graphicx}
%\usepackage[dvipdfmx]{graphicx}
%\usepackage{amsmath}
%\usepackage{amssymb}
%\usepackage{amsthm}
%\usepackage{mathrsfs}
%\newtheorem{dfn}{Definition}[section]
%\newtheorem{thm}[dfn]{Theorem}
%\newtheorem{prop}[dfn]{Proposition}
%\newtheorem{lem}[dfn]{Lemma}
%\newtheorem{cor}[dfn]{Corollary}
%\newtheorem{rem}[dfn]{Remark}
%\newtheorem{car}[dfn]{Computer Assisted Result}
%\newtheorem{ass}[dfn]{Assumption}
%\newtheorem{ex}[dfn]{Example}
%\newtheorem{nota}[dfn]{Notations}
%\newtheorem{alg}{Algorithm}
%\newtheorem{observation}[dfn]{Observation}
%\newtheorem{prob}[dfn]{Problem}
%\newtheorem{notation}[dfn]{Notation}
%\newtheorem{fact}[dfn]{Fact}
\newtheorem{conj}[dfn]{Conjecture}
%
%\newcommand{\Inv}{{\rm Inv}}
%\newcommand{\Int}{{\rm int}}
%\newcommand{\dir}{{\rm dir}}
%\newcommand{\Fix}{{\rm Fix}}
%\newcommand{\IH}{{\rm IH}}
%\newcommand{\Num}{{\rm Num}}
%\newcommand{\Ker}{{\rm Ker}}
%\newcommand{\Span}{{\rm span}}
%\newcommand{\Tube}{{\rm Tube}}
%\newcommand{\re}{{\rm Re}}
%\newcommand{\low}{{\rm low}}
%\newcommand{\err}{{\rm err}}
%\newcommand{\diag}{{\rm diag}}
%\newcommand{\diam}{{\rm diam}}
%\newcommand{\dist}{{\rm dist}}
%\newcommand{\sgn}{{\rm sgn}}
%\newcommand{\im}{{\rm Im}}
%\newcommand{\In}{{\rm in}}
%\newcommand{\Out}{{\rm out}}
%\newcommand{\exit}{{\rm exit}}
%\newcommand{\ent}{{\rm ent}}
%\newcommand{\dep}{{\rm dep}}
%\newcommand{\arr}{{\rm arr}}
%\newcommand{\Spec}{{\rm Spec}}
%
%\numberwithin{equation}{section}
%
%\setlength{\topmargin}{-30pt}
%\setlength{\oddsidemargin}{0.5cm}
%\setlength{\evensidemargin}{0.5cm}
%\setlength{\textwidth}{15cm}
%%\setlength{\textheight}{23.5cm}
%
%\newcommand{\KMa}[1]{{\color{black} #1}}
%\newcommand{\KMb}[1]{{\color{black} #1}}
%\newcommand{\KMc}[1]{{\color{black} #1}}
%
%\newcommand{\KMd}[1]{{\color{black} #1}}
%\newcommand{\KMe}[1]{{\color{black} #1}}
%\newcommand{\KMf}[1]{{\color{black} #1}}
%\newcommand{\KMfb}[1]{{\color{black} #1}}
%\newcommand{\KMg}[1]{{\color{black} #1}}
%\newcommand{\KMh}[1]{{\color{black} #1}}
%\newcommand{\KMi}[1]{{\color{black} #1}}
%\newcommand{\KMj}[1]{{\color{black} #1}}
%\newcommand{\KMk}[1]{{\color{black} #1}}
%\newcommand{\KMl}[1]{{\color{black} #1}}
%
%\usepackage{color}
%\begin{document}
%
%\title{Conjecture on the existence of maximizers}
%
%\author{Kaname Matsue \thanks{Institute of Mathematics for Industry / International Institute for Carbon-Neutral Energy Research (WPI-I$^2$CNER), Kyushu University, Fukuoka 819-0395, Japan, {\tt kmatsue@imi.kyushu-u.ac.jp} }}
%
%%\author{Hisatoshi Kodani\thanks{Advanced Institute for Materials Research, Tohoku University, 2-1-1 Katahira, Aoba-ku, Sendai, 980-8577, Japan ({\tt hisatoshi.kodani@tohoku.ac.jp})}, 
%%Kaname Matsue\thanks{(Corresponding author)} $^{,}$ \footnote{Institute of Mathematics for Industry, Kyushu University, Fukuoka 819-0395, Japan ({\tt kmatsue@imi.kyushu-u.ac.jp})} $^{,}$ \footnote{International Institute for Carbon-Neutral Energy Research (WPI-I$^2$CNER), Kyushu University, Fukuoka 819-0395, Japan} ,\\ 
%%Hiroyuki Ochiai\thanks{Institute of Mathematics for Industry, Kyushu University, Fukuoka 819-0395, Japan ({\tt ochiai@imi.kyushu-u.ac.jp})}
%%and Akitoshi Takayasu\thanks{Faculty of Engineering, Information and Systems, University of Tsukuba, 1-1-1 Tennodai, Tsukuba, Ibaraki 305-8573, Japan (\texttt{takitoshi@risk.tsukuba.ac.jp})}
%%}
%
%
%
%%\date{}
%\maketitle
%
%{\bf Keywords:} maximization of functionals, parameter dependence.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Main Results}
\label{results}

%====================================================
\subsection{Characterization for the scenario of a unique global maximizer}

Our first main theoretical result is given in the following theorem.

\begin{thm}
\label{thm-existence-max}
For {\bf any} configurations of given points $\mathcal{X}_n \equiv \{{\bf x}_i\}_{i=1}^n$, there is a positive number $h_0 = h_0(\mathcal{X}_n) > 0$ such that, for {\bf any} $h > h_0$, the functional $f({\bf x}, h)$ admits {\bf a unique global maximizer} ${\bf p} = {\bf p}(h, \mathcal{X}_n)$.
\end{thm}


First observe that, for any $h > 0$ as a parameter, $f({\bf x}, h)$ as a function of ${\bf x} = (x,y)$ is smooth on $\mathbb{R}^2$.
We therefore know that, for any local maximizer or minimizer ${\bf x}_\ast = (x_\ast, y_\ast)$ of $f$ must be critical points, namely
\begin{equation*}
\nabla_{\bf x} f({\bf x}, h) \equiv F({\bf x}, h) = \begin{pmatrix}
F_1({\bf x}, h) \\ F_2({\bf x}, h)
\end{pmatrix} = \begin{pmatrix}
0 \\ 0
\end{pmatrix}\quad \text{ at }\quad {\bf x} = {\bf x}_\ast. 
\end{equation*}
Our strategy for the proof of Theorem \ref{thm-existence-max} is decomposed into the following steps.
\begin{enumerate}
\item Maximizers or minimizers of $f$ must be located in a compact subset $R$ of $\mathbb{R}^2$.
As a result, $f$ admits at least one maximizer and minimizer.
\item The Jacobian matrix $D_{\bf x}F({\bf x},h)$ of $F$, namely the Hessian matrix ${\rm Hess}(f)({\bf x},h)$ of $f$ with respect to ${\bf x}$, is negative definite for all ${\bf x}\in R$, provided $h$ is sufficiently large. 
In particular, $f$ is strictly concave on $R$.
\end{enumerate}
%From these statements with several observations of $F$, the proof is completed.
Before starting the proof, observe that the gradient $F = \nabla_{\bf x} f$ at ${\bf p}=({\bf x},h)$ is given by
\begin{equation}
\label{grad-f}
F({\bf x}, h) = \begin{pmatrix}
F_1({\bf x}, h) \\ F_2({\bf x}, h)
\end{pmatrix} = \left( -m \sum_{i=1}^n \frac{x-x_i}{d_i^{m+2}},\quad -m \sum_{i=1}^n \frac{y-y_i}{d_i^{m+2}}\right)^T.
\end{equation}



%-------------------------------------------------------------------
\subsubsection{Step 1 in the proof of Theorem \ref{thm-existence-max}}
 
\begin{lem}
\label{lem-max-location}
Maximizers and minimizers of $f$ are located in the rectangular domain 
\begin{equation*}
R = R(\mathcal{X}_N) := \left[ \min_{i=1,\ldots, n} x_i, \max_{i=1,\ldots, n} x_i\right] \times \left[ \min_{i=1,\ldots, n} y_i, \max_{i=1,\ldots, n} y_i \right].
\end{equation*}
Moreover, $f$ does not attain a maximal value outside $R$.
\end{lem}
\begin{proof}
Let ${\bf x} = (x,y) \in \mathbb{R}^2\setminus R$.
Then, at least one the following cases must be held: (i) $x < x_i$ for all $i$, (ii) $x > x_i$ for all $i$, (iii) $y < y_i$ for all $i$, or (iv) $y > y_i$ for all $i$.
\par
When (i) holds, it follows from (\ref{grad-f}) that $F_1({\bf x},h) > 0$. 
Similarly, $F_1({\bf x},h) < 0$ must be satisfied when (ii) holds, while $F_2({\bf x},h) > 0$ when (iii) holds, and $F_2({\bf x},h) < 0$ when (iv) holds, respectively.
Because all local maximizers and minimizers must be critical points of $f$, namely zeros of $F$, the above assertions imply that any point ${\bf x} \in \mathbb{R}^2\setminus R$ must be neither a maximizer nor a minimizer of $f$.
\par
Finally, observations in cases (i) and (ii) also imply that $f$ must increase as $x$ moves toward
\begin{equation*}
R_x \equiv \left[ \min_{i=1,\ldots, n} x_i, \max_{i=1,\ldots, n} x_i\right],
\end{equation*}
the $x$-component of $R$.
The similar assertion holds for $y$, indicating that the maximizer ${\bf x}$ of $f$, if it exists, must be in $R$ and the proof is completed.
\end{proof}

Because our aim here is to find the global maximizer of $f$, we pay our attention to maximizers, which have to be in $R$.
Thanks to the smoothness of $f$ and the compactness of $R$, it admits at least one (local) maximizer in $R$.
The rest of our discussions here is the uniqueness.

%----------------------------------------------------------------------
\subsubsection{Step 2 in the proof of Theorem \ref{thm-existence-max}}

\begin{prop}
\label{prop-neg-def}
For any compact sets $K\subset \mathbb{R}^2$, there is a positive number $h_0 =h_0(K) > 0$ such that, for all $h > h_0$, $D_{\bf x}F({\bf x},h)$ is negative definite for all ${\bf x}\in K$.
\end{prop}

\begin{proof}[Proof of Proposition \ref{prop-neg-def}]
It is sufficient to prove that both eigenvalues of $D_{\bf x}F({\bf x},h)$ are negative for all ${\bf x} = (x,y)$ with a suitable choice of $h$.
Now the Jacobian matrix $D_{\bf x}F({\bf x},h)$ is given by
\begin{align*}
D_{\bf x}F({\bf x},h) &= \begin{pmatrix}
a & b \\ b & c
\end{pmatrix},\quad
%%%
a = -m  \sum_{i=1}^n \frac{1}{d_i^{m+2}}\left[ 1 - (m+2) \frac{(x - x_i)^2}{d_i^2}\right],\\ 
%
b &= m(m+2) \sum_{i=1}^n \frac{(x - x_i)(y - y_i)}{d_i^{m+4}}, \quad
%
c = -m  \sum_{i=1}^n \frac{1}{d_i^{m+2}}\left[ 1 - (m+2) \frac{(y - y_i)^2}{d_i^2}\right].
\end{align*}
Because $DF(x,y)$ is symmetric, both eigenvalues are real and hence it is sufficient to prove $a + c< 0$ and $ac > b^2$ for our statement.
\par
First observe that
\begin{align*}
a +c &= -m  \sum_{i=1}^n \frac{1}{d_i^{m+2}}\left[ 1 - (m+2) \frac{(x - x_i)^2}{d_i^2}\right] - m  \sum_{i=1}^n \frac{1}{d_i^{m+2}}\left[ 1 - (m+2) \frac{(y - y_i)^2}{d_i^2}\right] \\
	&= -m\sum_{i=1}^n \frac{1}{d_i^{m+2}} \left( 2 - (m+2) \frac{(x - x_i)^2 + (y - y_i)^2}{d_i^2}  \right).
\end{align*}
We easily know that the rightmost function is negative whenever
\begin{equation}
\label{ineq-1-i}
\frac{(x - x_i)^2 + (y - y_i)^2}{(x - x_i)^2 + (y - y_i)^2 + h^2} < \frac{2}{m+2}
\end{equation}
for all $i$.
For fixed ${\bf x}\in K$, we can choose $\tilde h_{0,i}^1 = \tilde h_{0,i}^1({\bf x})$ such that (\ref{ineq-1-i}) for all $h > \tilde h_{0,i}^1$.
Choosing $\tilde h_0^1({\bf x}) := \max_{i=1,\ldots, n}\tilde h_{0,i}^1({\bf x})$, the inequality (\ref{ineq-1-i}) holds for {\em all $i$} and all $h > \tilde h_0^1$, with fixed ${\bf x}\in K$.
By continuity of $a+c$ as a function of ${\bf x}$, we can choose an open neighborhood $U_{{\bf x}}\subset \mathbb{R}^2$ of ${\bf x}$ such that (\ref{ineq-1-i}) holds for all $i$, all $h > \tilde h_0^1$ and all $\tilde {\bf x} = (\tilde x,\tilde y)\in U_{{\bf x}}$.
By compactness of $K$, there is a finite subcovering $\{U_{{\bf x}_j'}\}_{j=1}^l$ of $K$ with $\{{\bf x}_j'\}_{j=1}^l \subset K$.
Therefore, letting
\begin{equation*}
h_0^1 := \max_{j=1,\ldots, l} \tilde h_0^1({\bf x}_j'),
\end{equation*}
it follows that the inequality (\ref{ineq-1-i}) holds for all $i$, all $h > h_0^1$ and {\em all ${\bf x}\in K$}.
\par
Next, observe that
\begin{align}
\notag
ac - b^2 &= \left( -m  \sum_{i=1}^n \frac{1}{d_i^{m+2}}\left[ 1 - (m+2) \frac{(x - x_i)^2}{d_i^2}\right]\right)\cdot \left( -m  \sum_{i=1}^n \frac{1}{d_i^{m+2}}\left[ 1 - (m+2) \frac{(y - y_i)^2}{d_i^2}\right] \right)\\
\notag
&\quad - m^2(m+2)^2 \left(\sum_{i=1}^n \frac{(x - x_i)(y - y_i)}{d_i^{m+4}}\right)^2\\
\notag
	&= m^2\left\{ \left( \sum_{i=1}^n \frac{1}{d_i^{m+2}}\left[ 1 - (m+2) \frac{(x - x_i)^2}{d_i^2}\right]\right)\cdot \left( \sum_{i=1}^n \frac{1}{d_i^{m+2}}\left[ 1 - (m+2) \frac{(y - y_i)^2}{d_i^2}\right] \right) \right.\\
\label{neg-2}
&\quad - \left. (m+2)^2 \left(\sum_{i=1}^n \frac{(x - x_i)(y - y_i)}{d_i^{m+4}}\right)^2 \right\}.
\end{align}
%%%
We shall estimate the rightmost function in (\ref{neg-2}) componentwise.
First we have
\begin{align}
\notag
&\frac{1}{d_i^{2(m+2)}}\left[ 1 - (m+2) \frac{(x - x_i)^2}{d_i^2}\right]\cdot \left[ 1 - (m+2) \frac{(y - y_i)^2}{d_i^2}\right] - (m+2)^2\frac{(x - x_i)^2(y - y_i)^2}{d_i^{2(m+4)}}\\
\label{neg-2-1}
&= \frac{1}{d_i^{2(m+2)}} \left\{ 1 - (m+2) \frac{(x - x_i)^2 + (y - y_i)^2}{d_i^2}\right\}.
\end{align}
and the right-hand side is estimated later.
Next consider
\begin{align*}
\frac{1}{d_i^{m+2}d_j^{m+2}}\left[ \left\{ 1 - (m+2) \frac{(x - x_i)^2}{d_i^2}\right\} \left\{ 1 - (m+2) \frac{(y - y_j)^2}{d_j^2}\right\}  +  \left\{ 1 - (m+2) \frac{(x - x_j)^2}{d_j^2}\right\} \left\{ 1 - (m+2) \frac{(y - y_i)^2}{d_i^2} \right\} \right] \\
- 2(m+2)^2\frac{(x - x_i)(y - y_i)}{d_i^{m+4}}\frac{(x - x_j)(y - y_j)}{d_j^{m+4}}
\end{align*}
with $i\not = j$.
Observe that
\begin{align*}
&\left\{ \frac{(x - x_i)^2}{d_i^2} \frac{(y - y_j)^2}{d_j^2} + \frac{(x - x_j)^2}{d_j^2} \frac{(y - y_i)^2}{d_i^2} \right\} - 2 \frac{(x - x_i)(y - y_i)}{d_i^2}\frac{(x - x_j)(y - y_j)}{d_j^2} \\
%%%
 &= \frac{1}{d_i^2d_j^2}\left\{ (x - x_i)^2 (y - y_j)^2 + (x - x_j)^2(y - y_i)^2 - 2(x - x_i)(y - y_i)(x - x_j)(y - y_j) \right\} \\
 &= \frac{1}{d_i^2d_j^2}\left\{ (x - x_i) (y - y_j) - (x - x_j)(y - y_i) \right\}^2 \geq 0.
\end{align*}
Then the rest is to estimate
\begin{align}
\label{neg-2-2}
2 - (m+2) \frac{(x - x_i)^2 + (y - y_i)^2}{d_i^2} - (m+2) \frac{(x - x_j)^2 + (y - y_j)^2}{d_j^2}.
\end{align}
Here it is concluded that both (\ref{neg-2-1}) and (\ref{neg-2-2}) are always satisfied whenever
\begin{equation}
\label{neg-2-3}
\frac{(x - x_i)^2 + (y - y_i)^2}{(x - x_i)^2 + (y - y_i)^2 + h^2} < \frac{1}{m+2},
\end{equation}
holds for all $i$.
The similar argument involving (\ref{ineq-1-i}) yields that the inequality (\ref{neg-2}) is true for all $h > \tilde h_{0,i}^2({\bf x})$ with some $\tilde h_{0,i}^2({\bf x}) > 0$.
Also, by the similar arguments to obtaining $h_0^1$, we know that there is a number $h_0^2 > 0$ such that (\ref{neg-2}) holds for all $i$, all $h > h_0^1$ and all ${\bf x}\in K$.
\par
Finally, choosing $h_0 := \max\{h_0^1, h_0^2\}$, we conclude that both inequalities $a + c < 0$ and $ac > b^2$ holds for all ${\bf x} \in K$ and all $h > h_0$, which proves our claim.
\end{proof}

Choosing $h_0$ with $K := R$ as in Proposition \ref{prop-neg-def} with $R$ defined in Lemma \ref{lem-max-location}, we know that
\begin{itemize}
\item $f$ has a (local) maximizer in $R$, and is strictly concave in $R$ in the sense that the Hessian matrix ${\rm Hess}(f)({\bf x})$ is negative definite for all ${\bf x}\in R$, whenever $h > h_0$,
\item $f$ does not attain maximal values outside $R$.
\end{itemize}
As a conclusion, the functional $f$ admits the unique global maximizer in $R$ and the proof of Theorem \ref{thm-existence-max} is completed.


%------------------------------------------------------------------------------
\subsection{Symmetry of functionals and possible maximizers: a case study }
\label{section-symmetry}

The previous arguments guarantee the {\em unique} existence of maximizers of $f$ when $h > 0$ is relatively large.
As seen below, there are possibilities to exist multiple (local) maximizers of $f$ when $h$ becomes considerably small.
In typical situations, the existence of multiple maximizers is a consequence of {\em bifurcations} of solutions to $F({\bf x},h) = 0$ and those bifurcations can be extracted through standard machineries in (numerical) bifurcation theory (e.g., \cite{K2013}).
On the other hand, when there are {\em symmetries} in our objects, multiple maximizers and/or their bifurcations can be considered. 
The simplest example to easily observe symmetry in our considering problem is the LED configuration, such as squares, hexahedra or circular distributions.
They possess reflection symmetry $(x, y)\mapsto (\pm x, \pm y)$ and/or rotations with fixed angle $\theta$:
\begin{equation}
\label{rotation}
\begin{pmatrix}
x \\ y
\end{pmatrix}\mapsto \begin{pmatrix}
\cos \theta & -\sin \theta \\ 
\sin \theta & \cos \theta
\end{pmatrix}\begin{pmatrix}
x \\ y
\end{pmatrix}.
\end{equation}
In addition to LED configurations, the functional $F = (F_1, F_2)$ should be paid attention to for extracting symmetry of maximizers.
Symmetry of $F$ can be restricted compared with that of LED configurations.
Here we discuss the possible symmetry on $F$ following the theory of {\em bifurcations with symmetry} (e.g., \cite{GSS1988}).
\par
\bigskip
Mathematically, symmetries on variables and functionals are described through {\em groups}. 
Let $\Gamma$ be a (compact Lie) group\footnote{
%	footnote
Our examples of $\Gamma$ are $\mathbb{Z}_n$ (cyclic group) or $D_n$ (dihedral groups) mentioned below.
Readers should not be worried much about the details of Lie groups.
%	footnote: end
}.
The {\em (linear) action of $\Gamma$ on the vector space $V$} is the mapping 
\begin{equation*}
\Gamma\times V\to V,\quad (\gamma, {\bf v}) \mapsto \gamma\cdot {\bf v}\quad ({\bf v}\in V)
\end{equation*}
such that:
\begin{enumerate}
\item For each $\gamma \in \Gamma$ the mapping $\rho_\gamma: V\to V$ defined by $\rho_\gamma({\bf v}) = \gamma\cdot {\bf v}$ is linear.
\item If $\gamma_1, \gamma_2 \in \Gamma$, then $\gamma_1\cdot (\gamma_2\cdot {\bf v}) = (\gamma_1\gamma_2)\cdot {\bf v}$.
\end{enumerate}
Examples of compact Lie groups exhibiting such actions are {\em cyclic groups} $\mathbb{Z}_n$ or {\em dihedral groups} $D_n$ for some integer $n$.
Several actions of these groups we shall frequently use here are the following:
\begin{description}
\item[$\mathbb{Z}_2$-actions on $\mathbb{R}^2$.]
\end{description}
Either of them:
\begin{equation*}
\begin{pmatrix}
x \\ y
\end{pmatrix}\mapsto \begin{pmatrix}
-x \\ y
\end{pmatrix},\quad 
%%%
\begin{pmatrix}
x \\ y
\end{pmatrix}\mapsto \begin{pmatrix}
x \\ -y
\end{pmatrix},\quad
\begin{pmatrix}
x \\ y
\end{pmatrix}\mapsto \begin{pmatrix}
-x \\ -y
\end{pmatrix},
\end{equation*}
namely {\em reflection} in one axis or two axes simultaneously.
\begin{description}
\item[A $D_n$-action on $\mathbb{R}^2$.]
\end{description}
The following transformations and their compositions:
\begin{equation}
\label{Dn} 
\xi_n: \begin{pmatrix}
x \\ y
\end{pmatrix}\mapsto \begin{pmatrix}
\cos \frac{2\pi}{n} & -\sin \frac{2\pi}{n} \\ 
\sin \frac{2\pi}{n} & \cos \frac{2\pi}{n}
\end{pmatrix}\begin{pmatrix}
x \\ y
\end{pmatrix},\quad 
%%%
\kappa: \begin{pmatrix}
x \\ y
\end{pmatrix}\mapsto \begin{pmatrix}
x \\ -y
\end{pmatrix},
\end{equation}
namely reflection and {\em rotation}.


\begin{dfn}\rm
Let $\Gamma$ be a (compact Lie) group acting linearly on a vector space $V$, and $g: V\to V$ be a mapping.
We say that $g$ is {\em $\Gamma$-equivariant} if
\begin{equation*}
g(\gamma \cdot {\bf v}) = \gamma \cdot g({\bf v})
\end{equation*}
holds for all $\gamma \in \Gamma$ and ${\bf v}\in V$.
\end{dfn}


We concentrate on the most symmetric case in $\mathbb{R}^2$ with discretely distributed configurations; the {\em circular} configuration.
In the following proposition, labeling of the LED configuration is changed for easier expressions of points and their images of actions.
\begin{prop}
\label{prop-equivariant-LED}
Let $\mathcal{X}_n = \{{\bf x}_i\}_{i=0}^{n-1} \subset \mathbb{R}^2$ be the LED configuration evenly distributed on a circle with radius $r > 0$.
Define the $D_n$-action on $\mathbb{R}^2$ by (\ref{Dn}).
Then, for all $h>0$, the functional $F$ is $D_n$-equivariant in ${\bf x}$.
\end{prop}

\begin{proof}
Without the loss of generality, we may fix the position of each LED ${\bf x}_k$, $k=0,\ldots, n-1$ as
\begin{equation*}
{\bf x}_k \equiv (x_k, y_k)^T = \left( r\cos (kw_n), r\sin (kw_n) \right)^T,\quad w_n = \frac{2\pi}{n}.
\end{equation*}
Now the dihedral group $D_n$ generated by transformations (\ref{Dn}) is acting on $\mathbb{R}^2$, and the configuration $\mathcal{X}_n$ is $D_n$-invariant in the sense that, for any $\gamma\in D_n$ and ${\bf x}\in \mathcal{X}_n$, there is $\tilde {\bf x}\in \mathcal{X}_n$ such that $\gamma\cdot {\bf x} = \tilde {\bf x}$.
It is sufficient to show that 
\begin{equation*}
(F_1(\gamma\cdot {\bf x}, h), F_2(\gamma\cdot {\bf x}, h)) = \gamma\cdot (F_1({\bf x}, h), F_2({\bf x}, h))
\end{equation*}
for any $h > 0$ when $\gamma = \xi_n, \kappa$ given in (\ref{Dn}), thanks to the definition of the $D_n$-action on $\mathbb{R}^2$.
\par
First consider the action $\kappa$; the reflection across the $x$-axis.
Direct calculations yield that ${\bf x}\in \mathcal{X}_n$ if and only if $\kappa\cdot {\bf x}\in\mathcal{X}_n$.
More precisely, for ${\bf x} = {\bf x}_k$, the reflection $\kappa\cdot {\bf x}$ is given by ${\bf x}_{n-k}$ with the identification ${\bf x}_{n} = {\bf x}_0$.
We shall always use this identification unless otherwise noted.
Let ${\bf x} = (x,y)\in \mathbb{R}^2$ and consider the $\mathbb{Z}_2$-action given by
\begin{equation*}
\kappa: (x, y)^T \mapsto (x, -y)^T.
\end{equation*}
Then
\begin{align*}
F(x, -y, h) &= (F_1(x, -y, h), F_2(x, -y, h)),\\
\frac{-1}{m}F_1(x, -y, h) &= \sum_{i=0}^{n-1} \frac{x-x_i}{\{(x - x_i)^2 + (-y - y_i)^2 + h^2\}^{(m+2)/2}}\\
	&= \frac{x- 1}{\{(x - 1)^2 + y^2 + h^2\}^{(m+2)/2}} + \sum_{i=1}^{n-1} \frac{x-x_i}{\{(x - x_i)^2 + (-y - y_i)^2 + h^2\}^{(m+2)/2}}\\
	&= \frac{x- 1}{\{(x - 1)^2 + y^2 + h^2\}^{(m+2)/2}} + \sum_{i=1}^{n-1} \frac{x-x_i}{\{(x - x_i)^2 + (y + y_i)^2 + h^2\}^{(m+2)/2}}\\
	&= \frac{x- 1}{\{(x - 1)^2 + y^2 + h^2\}^{(m+2)/2}} + \sum_{i=1}^{n-1} \frac{x-x_{n-i}}{\{(x - x_{n-i})^2 + (y- y_{n-i})^2 + h^2\}^{(m+2)/2}}\\
	&= \sum_{i=0}^{n-1} \frac{x-x_i}{\{(x - x_i)^2 + (-y - y_i)^2 + h^2\}^{(m+2)/2}},
\end{align*}
while
\begin{align*}
\frac{-1}{m}F_2(x, -y, h) &= \sum_{i=0}^{n-1} \frac{-y-y_i}{\{(x - x_i)^2 + (-y - y_i)^2 + h^2\}^{(m+2)/2}}\\
	&= \frac{-y}{\{(x - 1)^2 + y^2 + h^2\}^{(m+2)/2}} + \sum_{i=1}^{n-1} \frac{-y-y_i}{\{(x - x_i)^2 + (-y - y_i)^2 + h^2\}^{(m+2)/2}}\\
	&= \frac{x- 1}{\{(x - 1)^2 + y^2 + h^2\}^{(m+2)/2}} + \sum_{i=1}^{n-1} \frac{-y-y_i}{\{(x - x_i)^2 + (y + y_i)^2 + h^2\}^{(m+2)/2}}\\
	&= \frac{x- 1}{\{(x - 1)^2 + y^2 + h^2\}^{(m+2)/2}} + \sum_{i=1}^{n-1} \frac{-y+y_{n-i}}{\{(x - x_{n-i})^2 + (y- y_{n-i})^2 + h^2\}^{(m+2)/2}}\\
	&= - \sum_{i=0}^{n-1} \frac{y-y_i}{\{(x - x_i)^2 + (-y - y_i)^2 + h^2\}^{(m+2)/2}}.
\end{align*}
Consequently, we have $F(\kappa\cdot {\bf x}, h) = \kappa F({\bf x}, h) = (F_1({\bf x}, h), -F_2({\bf x}, h))$, i.e., $F$ is $\mathbb{Z}_2$-equivariant in ${\bf x}$.
Note that the group $\mathbb{Z}_2$ generated by $\kappa$ is a subgroup of $D_n$.
\par
Next consider the action $\xi_n$; the $w_n$-rotation.
For given ${\bf x}= (x,y)^T\in \mathbb{R}^2$, let $\tilde {\bf x} = \xi_n\cdot {\bf x} \equiv (\tilde x, \tilde y)$.
More precisely,
\begin{equation*}
\tilde x = (\cos w_n)x - (\sin w_n)y \equiv c_n x - s_n y,\quad 
\tilde y = (\sin w_n)x + (\cos w_n)y \equiv s_n x + c_n y.
\end{equation*}
First observe that the summand theorem for trigonometric functions indicates that
\begin{align*}
x_i &= r\cos (iw_n) = r\cos \{(i-1)w_n + w_n\} = r\{\cos (i-1)w_n\} \cos w_n - r\{\sin (i-1)w_n\} \sin w_n\\ 
	&= x_{i-1}c_n - y_{i-1}s_n,\\
y_i &= r\sin (iw_n) = r\sin \{(i-1)w_n + w_n\} = r\{\sin (i-1)w_n \} \cos w_n + r\{\cos (i-1)w_n\} \sin w_n\\
	&= y_{i-1}c_n + x_{i-1}s_n.
\end{align*}
Using these identifications, we have
\begin{align}
\notag
\tilde x - x_i &= (\cos w_n)x - (\sin w_n)y - x_i
	= c_n x - s_n y - \{ x_{i-1}c_n - y_{i-1}s_n \} \\
\notag
	&= c_n (x - x_{i-1}) - s_n (y - y_{i-1}),\\
%%%
\notag
\tilde y - y_i &= (\sin w_n)x + (\cos w_n)y - y_i
\notag
	= s_n x + c_n y - \{ y_{i-1}c_n + x_{i-1}s_n \}\\
\label{identity-tri}
	&= s_n(x - x_{i-1}) + c_n (y - y_{y-1}).
\end{align}
Now
\begin{align*}
F(\tilde {\bf x}, h) &= (F_1(\tilde {\bf x}, h), F_2(\tilde {\bf x}, h)),\\
\frac{-1}{m}F_1(\tilde {\bf x}, h) &= \sum_{i=0}^{n-1} \frac{(\cos w_n)x - (\sin w_n)y -x_i}{\{ \{ (\cos w_n)x - (\sin w_n)y - x_i\}^2 + \{ (\sin w_n)x + (\cos w_n)y - y_i\}^2 + h^2\}^{(m+2)/2}},
\end{align*}
while
\begin{equation*}
\frac{-1}{m}F_2(\tilde {\bf x}, h) = \sum_{i=0}^{n-1} \frac{(\sin w_n)x + (\cos w_n)y -y_i}{\{ \{ (\cos w_n)x - (\sin w_n)y - x_i\}^2 + \{ (\sin w_n)x + (\cos w_n)y - y_i\}^2 + h^2\}^{(m+2)/2}}.
\end{equation*}
From (\ref{identity-tri}), we have
\begin{align*}
\{(\cos w_n)x - (\sin w_n)y -x_i\}^2 &= \{c_n (x - x_{i-1}) - s_n (y - y_{i-1})\}^2\\
	&= c_n^2 (x - x_{i-1})^2 -2c_n s_n(x - x_{i-1}) (y - y_{i-1}) + s_n^2 (y - y_{i-1})^2,\\
 \{ (\sin w_n)x + (\cos w_n)y - y_i\}^2 &= \{y_1(x - x_{i-1}) + x_1 (y - y_{y-1})\}^2 \\
 	&= s_n^2 (x - x_{i-1})^2 + 2c_n s_n (x - x_{i-1}) (y - y_{i-1}) + c_n^2 (y - y_{i-1})^2,\\
S &\equiv \{(\cos w_n)x - (\sin w_n)y -x_i\}^2 +  \{ (\sin w_n)x + (\cos w_n)y - y_i\}^2\\
	&= (c_n^2 + s_n^2)(x - x_{i-1})^2 + (s_n^2 + c_n^2)  (y - y_{i-1})^2\\
	&= (x - x_{i-1})^2 + (y - y_{i-1})^2
\end{align*}
and hence, writing $d_i^2 \equiv (x - x_i)^2 + (y - y_i)^2 + h^2$, we know that
\begin{align*}
\frac{-1}{m}F_1(\tilde {\bf x}, h) &= \sum_{i=0}^{n-1} \frac{(\cos w_n)x - (\sin w_n)y -x_i}{ d_i ^{(m+2)/2}} \\
	&=  \sum_{i=0}^{n-1} \frac{ c_n (x - x_{i-1}) - s_n (y - y_{i-1}) }{ d_{i-1}^{(m+2)/2} }\\
	&= c_n F_1({\bf x}, h) - s_n F_2({\bf x}, h), \\
\frac{-1}{m}F_2(\tilde {\bf x}, h) &= \sum_{i=0}^{n-1} \frac{(\sin w_n)x + (\cos w_n)y -x_i}{ d_i^{(m+2)/2}} \\
&= \sum_{i=0}^{n-1} \frac{ s_n (x - x_{i-1}) + c_n (y - y_{y-1}) }{ d_{i-1}^{(m+2)/2}} \\
	&= s_n F_1({\bf x}, h) + c_n F_2({\bf x}, h),
\end{align*}
where we have identified $d_{-1}$ with $d_{n-1}$.
As a consequence, we have $F(\xi_n\cdot {\bf x}, h) = \xi_n \cdot F({\bf x}, h)$ for all ${\bf x}\in \mathbb{R}^2$ and hence the equivariance is verified.
\end{proof}

The above arguments provide a strategy to find equivariance of $F$ associated with a group $\Gamma$ with different LED configurations, such as square-, or rectangular-like ones.
\par
\bigskip
From the equivariance of $F$, we can consider the bifurcation problem for $F$ with the height $h > 0$ as the bifurcation parameter as that with the symmetry $D_n$.
According to the general theory \cite{GSS1988}, symmetry breaking bifurcations {\em generically}\footnote{
%	footnote
Detailed meaning of this concept is written in \cite{GSS1988}.
%	footnote: end
} occur following {\em isotropy subgroups}.
\begin{dfn}\rm
Let $\Gamma$ be a (compact Lie) group acting on a vector space $V$.
The {\em isotropy subgroup} of ${\bf x}\in V$ is
\begin{equation}
\Sigma_{\bf x} = \{\gamma \in \Gamma \mid \gamma \cdot {\bf x} = {\bf x} \}.
\end{equation}
Next, let $\Sigma \subset \Gamma$ be a subgroup.
The {\em fixed-point subspace} of $\Sigma$ is 
\begin{equation*}
{\rm Fix}(\Sigma) = \{{\bf x} \in V \mid \sigma \cdot {\bf x} = {\bf x} \text{ for all }\sigma \in \Sigma\}.
\end{equation*}
Finally, the action of $\Gamma$ on $V$ is said to be {\em absolutely irreducible} if the only linear mappings on $V$ that commute with either $\Gamma$ are scalar multiples of the identity.
\end{dfn}

The general theory in \cite{GSS1988} shows that the dihedral group $D_n$ includes $\mathbb{Z}_2$ as, up to isomorphisms,  the only (and maximal) isotropy subgroups, while the precise description of these subgroups is mentioned later. 
Maximality of an isotropic subgroup $\Sigma$ means that, if $\tilde \Sigma$ is an isotropic subgroup of $\Gamma$ properly containing $\Sigma$, then $\tilde \Sigma = \Gamma$.
\par
We can apply the {\em equivariant branching lemma} mentioned in \cite{GSS1988} Chapter XIII-3 stating as follows to characterizing symmetry-breaking structures in the bifurcation problem $F = F(\cdot, h) = 0$.

\begin{thm}[Equivariant branching lemma, \cite{GSS1988}]
\label{thm-branching}
Let $\Gamma$ be a Lie group acting absolutely irreducibly on a vector space $V$ and let $g = g({\bf x}, h)$ be a $\Gamma$-equivariant bifurcation problem satisfying
\begin{equation}
\label{absolute-g}
(D_{\bf x}g)_{{\bf 0}, h} = c(h) I\quad \text{ with }\quad c(h_0) = 0,\quad c'(h_0)\not = 0.
\end{equation}
Let $\Sigma$ be an isotropy subgroup satisfying 
\begin{equation*}
\dim {\rm Fix}(\Sigma) = 1.
\end{equation*}
Then there exists a unique smooth solution branch to $g = 0$ such that the isotropy subgroup of each solution is $\Sigma$.
\end{thm}


\begin{rem}[\cite{GS2002}, Chapter I]
The (maximal) isotropic subgroups $\mathbb{Z}_2$ of $D_n$ acting on $\mathbb{R}^2$ are characterized as follows.
The simplest isotropic subgroup is 
\begin{equation*}
\Sigma = \mathbb{Z}_2(\kappa) \equiv \{1, \kappa\}, \kappa: \begin{pmatrix}
x \\ y
\end{pmatrix}\mapsto \begin{pmatrix}
x \\ -y
\end{pmatrix},
\end{equation*}
i.e., the reflection symmetry. 
Because we are interested in $D_n$-action on $\mathbb{R}^2$, then the fixed-point subspace of $\Sigma$ is 
\begin{equation*}
{\rm Fix}(\Sigma) = \{(x,0) \in \mathbb{R}^2\} \cong \mathbb{R}.
\end{equation*}
Therefore $\Sigma = \mathbb{Z}_2(\kappa)$ satisfies the requirement stated in Theorem \ref{thm-branching}.
In general, as mentioned in \cite{GS2002}, group related solutions have {\em conjugate} isotropy subgroups.
Indeed, if $g({\bf x}, h) = 0$ for the $\Gamma$-equivariant map $g = g(\cdot, h)$ for any fixed parameter $h$, then $g(\gamma\cdot {\bf x}, h) = \gamma g({\bf x}, h) = 0$ for any $\gamma \in \Gamma$.
Now suppose that $\sigma \cdot {\bf x} = {\bf x}$, namely $\sigma$ is an element of the isotropy subgroup $\Sigma_{\bf x}$.
Then we have
\begin{equation*}
(\gamma \circ \sigma \circ \gamma^{-1})\gamma \cdot {\bf x} = (\gamma \circ \sigma) \cdot {\bf x} = \gamma \cdot {\bf x}.
\end{equation*}
This implies that the following {\em conjugacy} relation between isotropic subgroups holds:
\begin{equation*}
\Sigma_{\gamma \cdot {\bf x}} = \gamma \Sigma_{\bf x} \gamma^{-1} \equiv \{ \gamma \circ \sigma \circ \gamma^{-1}\mid \sigma \in \Sigma_{\bf x}\}.
\end{equation*}
Also, if $T = \gamma \Sigma \gamma^{-1}$, then we have ${\rm Fix}(T) = \gamma ({\rm Fix}(\Sigma))$.
In particular, $\dim {\rm Fix}(T) = 1$ if $\dim {\rm Fix}(\Sigma) = 1$ and hence we have the conjugate class of $1$-dimensional isotropic subgroups.
\par
When $n$ is odd, any power of the rotation action $\xi_n^k$ on $D_n$ does not coincide with the reflection $\kappa$, indicating that the reflection symmetry group $\mathbb{Z}_2(\kappa)$ admits exactly $n$ conjugate groups $\{\mathbb{Z}_2(\kappa \circ \xi_n^k)\}_{k=0}^{n-1}$, all of which admits $1$-dimensional fixed-point subspaces:
\begin{equation}
\label{fix-odd}
{\rm Fix}(\mathbb{Z}_2(\kappa \circ \xi_n^k)) = \left\{ \left(x\cos \frac{k\pi}{n}, -x\sin \frac{k\pi}{n} \right) \mid  x \in \mathbb{R} \right\}.
\end{equation}
When $n$ is even, on the other hand, the reflection symmetry $\kappa$ coincides with the $\pi$-rotation symmetry $\xi_n^{n/2}\equiv R_{\pi/2}$.
Therefore the subgroups conjugate to $\mathbb{Z}_2(\kappa)$ are written by 
\begin{equation*}
\mathbb{Z}_2(\kappa \circ \xi_n^k)\quad \left(k=0,1,\ldots, \frac{n}{2}-1\right),\quad \mathbb{Z}_2(\kappa \circ R_{\pi/2} \circ \xi_n^k)\quad \left(k=0,1,\ldots, \frac{n}{2}-1\right), 
\end{equation*}
while fixed-point subspaces are described by
\begin{equation}
\label{fix-even}
\left\{ \left(x\cos \frac{k\pi}{n}, -x\sin \frac{k\pi}{n} \right) \mid  x \in \mathbb{R} \right\},
\end{equation}
for any $k = 0,\ldots, n-1$.
%%%
% includes the group $\mathbb{Z}_2 = \mathbb{Z}_2(\kappa)$ generated by $\kappa$ given in (\ref{Dn}) as the only maximal isotropy subgroups, while $D_n$ with even $n$ includes the groups $\mathbb{Z}_2({\color{red}\tilde \kappa^k})$ with different generators ${\color{red}\tilde \kappa^k = \kappa_y \circ \xi_n^k}$ determined by 
%\begin{equation*}
%{\color{red}  \begin{pmatrix}
%x \\ y
%\end{pmatrix}\mapsto \begin{pmatrix}
%\cos \frac{2k\pi}{n} x -\sin \frac{2k\pi}{n}y \\ 
%\sin \frac{2k\pi}{n} x + \cos \frac{2k\pi}{n}y
%\end{pmatrix}\equiv \xi_n^k \cdot \begin{pmatrix}
%x \\ y
%\end{pmatrix}\mapsto\begin{pmatrix}
%\cos \frac{2k\pi}{n} x -\sin \frac{2k\pi}{n}y \\ 
%- \sin \frac{2k\pi}{n} x - \cos \frac{2k\pi}{n}y
%\end{pmatrix} \equiv }
%\end{equation*}
%as the maximal isotropy subgroups.
\end{rem}


Here we pay our attention to $\mathcal{X}_n = \{{\bf x}_i\}_{i=0}^{n-1} \subset \mathbb{R}^2$ with $n\geq 3$, the LED configuration considered in Proposition \ref{prop-equivariant-LED}.
Now suppose that one LED ${\bf x}_i \in \mathcal{X}_n$ is on the $x$-axis.
We then observe from the above arguments that
\begin{itemize}
\item $F$ is $D_n$-equivariant generated by (\ref{Dn}) (Proposition \ref{prop-equivariant-LED});
\item ${\rm Fix}(D_n) = \{{\bf 0}\}$,
\item for any $n$, $\mathbb{Z}_2(\kappa \circ \xi_n^k)$, $k=0,\cdots, n-1$, are maximal isotropic subgroups of $D_n$ whose fixed-point subspaces are one-dimensional.
\end{itemize}

We shall observe in Section \ref{section-numerical-bifurcation} that there is a critical $h = h_0 > 0$ such that the Jacobian matrix $D_{\bf x}F({\bf 0}, h_0)$ is the zero matrix, while $D_{\bf x}F({\bf 0}, h)$ has double (in particular, identical) eigenvalues, which indicates that the action $D_n$ on $\mathbb{R}^2$ is absolutely irreducible and (\ref{absolute-g}) holds for $D_{\bf x}F({\bf 0}, h)$.
%%%
Theorem \ref{thm-branching} then provides the existence of the smooth curve of solutions bifurcated from the origin ${\bf 0} =(0,0)^T$ whose isotropic subgroups are determined by the above conjugate class of isotropic subgroups.
In particular, the following consequences hold:

\begin{itemize}
\item for any $n$, there is the locally unique smooth curve of solutions starting from the origin ${\bf 0} =(0,0)^T$ running on the $x$-axis;
\item there are also locally unique smooth curve of solutions starting from the origin ${\bf 0} =(0,0)^T$ running on the fixed-point subspaces (\ref{fix-odd}) or (\ref{fix-even}) for $k=1,\ldots, n-1$.
\end{itemize}
Note that, when $n$ is even, there are two bifurcated solutions to $F(\cdot, h) = 0$ on the fixed-point subspaces due to the coincidence of $\kappa$ and the $\pi$-rotation symmetry $R$. 
The most important point is that the above scenario is {\em the only possible} bifurcation from the origin at a bifurcation point for the evenly distributed circular LED configuration.
Note again that the above structure is intrinsically determined by {\em isotropic subgroups} of a Lie group $\Gamma$ acting on $\mathbb{R}^2$ and the functional $F$ being $\Gamma$-equivariant.
The similar arguments to the above ones will provide the corresponding bifurcation structures of maximizers in the other configurations.

\par
\bigskip
Finally note that, as far as the bifurcation structure for $D_n$-symmetry is generated following Theorem \ref{thm-branching}, there is {\em no} possibility of the presence of bifurcations with rotational symmetry breaking.
Indeed, $D_n$ does not contain the cyclic group $\mathbb{Z}_n$ (describing rotation symmetry) as an isotropy subgroup except the origin.
Even if the isotropy subgroup including rotational symmetry, which is $\Sigma = \Sigma_{{\bf 0}} = D_n$, the fixed-point subspace is $0$-dimensional, which is incompatible with the situation in Theorem \ref{thm-branching}.




